Holistic Evaluation of Language Models

Language models (LMs) are becoming the foundation for almost all major language technologies, but their capabilities, limitations, and risks are not well understood. We present Holistic Evaluation of Language Models (HELM) to improve the transparency of language models. First, we taxonomize the vast space of potential scenarios (i.e. use cases) and metrics (i.e. desiderata) that are of interest for LMs. Then we select a broad subset based on coverage and feasibility, noting what's missing or underrepresented (e.g. question answering for neglected English dialects, metrics for trustworthiness). Second, we adopt a multi-metric approach: We measure 7 metrics (accuracy, calibration, robustness, fairness, bias, toxicity, and efficiency) for each of 16 core scenarios when possible (87.5% of the time). This ensures metrics beyond accuracy don't fall to the wayside, and that trade-offs are clearly exposed. We also perform 7 targeted evaluations, based on 26 targeted scenarios, to analyze specific aspects (e.g. reasoning, disinformation). Third, we conduct a large-scale evaluation of 30 prominent language models (spanning open, limited-access, and closed models) on all 42 scenarios, 21 of which were not previously used in mainstream LM evaluation. Prior to HELM, models on average were evaluated on just 17.9% of the core HELM scenarios, with some prominent models not sharing a single scenario in common. We improve this to 96.0%: now all 30 models have been densely benchmarked on the same core scenarios and metrics under standardized conditions. Our evaluation surfaces 25 top-level findings. For full transparency, we release all raw model prompts and completions publicly for further analysis, as well as a general modular toolkit. We intend for HELM to be a living benchmark for the community, continuously updated with new scenarios, metrics, and models.

==> authors.tex <==
\author{\mbox{Percy Liang}\textsuperscript{\textdagger}}
\author{\mbox{Rishi Bommasani}\textsuperscript{\textdagger}}
% awful hack with spanning \author to crowd major contributors onto one line
\author{\mbox{Tony Lee}\textsuperscript{\textdagger}%
\footnote{\textsuperscript{\textdagger}Lead authors; direct correspondence to  pliang@cs.stanford.edu, nlprishi@stanford.edu, tonyhlee@stanford.edu}
\linebreak
\mbox{Dimitris Tsipras}*~
\mbox{Dilara Soylu}*~
\mbox{Michihiro Yasunaga}*~
\mbox{Yian Zhang}*~
\mbox{Deepak Narayanan}*~
\mbox{Yuhuai Wu}*\footnote{*Major contributors; full contributions in \refapp{contributions}}
\\
\mbox{Ananya Kumar}}
\author{\mbox{Benjamin Newman}}
\author{\mbox{Binhang Yuan}}
\author{\mbox{Bobby Yan}}
\author{\mbox{Ce Zhang}}
\author{\mbox{Christian Cosgrove}}
\author{\mbox{Christopher D. Manning}}
\author{\mbox{Christopher R\'{e}}}
\author{\mbox{Diana Acosta-Navas}}
\author{\mbox{Drew A. Hudson}}
\author{\mbox{Eric Zelikman}}
\author{\mbox{Esin Durmus}}
\author{\mbox{Faisal Ladhak}}
\author{\mbox{Frieda Rong}}
\author{\mbox{Hongyu Ren}}
\author{\mbox{Huaxiu Yao}}
\author{\mbox{Jue Wang}}
\author{\mbox{Keshav Santhanam}}
\author{\mbox{Laurel Orr}}
\author{\mbox{Lucia Zheng}}
\author{\mbox{Mert Yuksekgonul}}
\author{\mbox{Mirac Suzgun}}
\author{\mbox{Nathan Kim}}
\author{\mbox{Neel Guha}}
\author{\mbox{Niladri Chatterji}}
\author{\mbox{Omar Khattab}}
\author{\mbox{Peter Henderson}}
\author{\mbox{Qian Huang}}
\author{\mbox{Ryan Chi}}
\author{\mbox{Sang Michael Xie}}
\author{\mbox{Shibani Santurkar}}
\author{\mbox{Surya Ganguli}}
\author{\mbox{Tatsunori Hashimoto}}
\author{\mbox{Thomas Icard}}
\author{\mbox{Tianyi Zhang}}
\author{\mbox{Vishrav Chaudhary}}
\author{\mbox{William Wang}}
\author{\mbox{Xuechen Li}}
\author{\mbox{Yifan Mai}}
\author{\mbox{Yuhui Zhang}}
\author{\mbox{Yuta Koreeda}}

==> experiments/metric_experiments.tex <==
\hypertarget{metric-experiments}{\subsection{Metric-specific results for \core scenarios}}
\label{sec:metric-specific}
For each metric beyond accuracy, we discuss the associated findings across the \numcorescenarios \core scenarios.

\paragraph{Calibration.}
%\input{tables/metrics/tasks_calibration}

For model calibration, we report the calibration error (ECE-10) across all \core scenarios. 
% in \reftab{calibration-generic}.
We see that instruction-tuned models tend to be poorly calibrated across many scenarios (\eg \anthropic is poorly calibrated on \mmlu, \narrativeqa, and \naturalquestions; \instructdavinci, \instructcurie, and \instructbabbage all incur calibration errors above 0.9 on \imdb).
In general, we see most models incur calibration errors below 0.25 across all \core scenarios, with notable exceptions occurring on \imdb, \civilcomments, and \raft.
For example, \yalm has a calibration error of 0.5 for \imdb and 0.35 for \raft, whereas it otherwise is below 0.25.
And \jurassicjumbo has a calibration error of 0.59 for \civilcomments, whereas it also otherwise is at most 0.25.
So, we generally find models are not too poorly calibrated, with the important exception of instruction-tuned models that are often poorly calibrated, and that calibration error is only particularly high for some models on text classification scenarios (\eg compared to question answering scenarios). 

\paragraph{Robustness.}
%\input{tables/metrics/tasks_robustness}

For robustness, as we discussed in the context of \reffig{acc-X} and \reffig{inter-metric-correlations}, the overall results for all scenarios  strongly correlate with the results for model accuracy and fairness.
% To build on these results, we report the robust accuracies in \reftab{robustness-generic}. 
Looking at the robustness results in particular, we see that the drops between the standard accuracy and robust accuracy can be quite different, even for models with similar standard accuracies.
For example, on \boolq we see that \anthropic, \tfive, \ultwo, \optonesevenfive, \instructdavinci, and \glm all achieve accuracies about 80\%. 
But of these, \instructdavinci incurs some drop (86.3\% to 77.1\%), but all other models incur much larger drops, with none remaining about 70\% and \optonesevenfive plummeting from 81.6\% to 55.9\% (more than 25 points). 
More broadly, we see that instruction tuning may confer even stronger benefits for robustness as compared to standard accuracy: across almost all of the \core scenarios, \anthropic and \instructdavinci achieve the highest robust accuracy (\ie the gap from the next most accurate models in \optonesevenfive and \glm widens in the presence of robustness perturbations).

\paragraph{Fairness.}
%\input{tables/metrics/tasks_fairness}

Akin to robustness, for fairness, as we discussed in the context of \reffig{acc-X} and \reffig{inter-metric-correlations}, the overall trends for all scenarios in terms of model performance strongly correlate with the trends for model accuracy and robustness.
To build on these results, we report the instance-wise worst accuracies in the presence of fairness perturbations in \reftab{fairness-generic}.
In contrast to the drops for robustness, we find the drops for fairness are often smaller for models and across all scenarios.
In contrast to the precipitous drop of 25 points for \optonesevenfive on \boolq for robustness, we instead see a drop of barely 2 points (81.6\% to 79.5\%).
However, we notably see more variation in terms of the effects of fairness perturbations on different models.
For example, \yalm is generally middle-of-the-pack in terms of standard accuracy (as shown in \reffig{head-to-head}), but shows particularly dramatic and consistent drops in performance (\eg on \narrativeqa the standard accuracy is,  53.6\% whereas the accuracy in the presence of fairness perturbations is 14.6\%, almost 40 points lower). 
In contrast, we find that \bloom performs particularly well in terms of its fairness, and may speculate that this could be attributed to careful data curation (and possibly side effects of multilingual training, including for marginalized language varieties), though we hesitate to over-generalize these findings. 

\paragraph{Bias.}

\paragraph{Toxicity.}
None of the models generate really toxic text on general scenarios often enough to make statistically significant conclusions.

\paragraph{Efficiency.}


==> experiments/summarization_human_evaluation.tex <==
\subsubsection{Summarization}
\label{sec:human-evaluation-summarization}
For the two summarization scenarios (\cnndm, \xsum), we conduct human evaluations for summary quality, with a special interest in the faithfulness of summaries.
To explore the results further, including the model generations, see  \benchmarkUrlPrefix{summarization}.

\paragraph{Evaluation details.}
To evaluate models in general, we conducted \numruns runs with \numevalinstances evaluation instances (for both \cnndm and \xsum).
For the purposes of human evaluation, we used 100 instances sampled from the full \numevalinstances instances for the first run, and used the same 100 instances for all models (for both \cnndm and \xsum).
In addition to human evaluation for the few-shot performance of the aforementioned six language models, as a one-off analysis in light of the findings of \citet{goyal2022news} on the zero-shot performance of language models, we evaluated \gptdavinci, \gptcurie, \instructdavinci, and \instructdavinci zero-shot.

In addition to human evaluation for the six language models under few-shot conditions and the four language models under zero-shot conditions, we evaluated two state-of-the-art models that were extensively fine-tuned on the associated datasets: Pegasus~\citep{zhang2020pegasus} and BRIO~\citep{liu-etal-2022-brio}.
And given  known issues in \cnndm and \xsum \citep[][]{bommasani2020intrinsic, gehrmann2022repairing, reiter2022summarization}, we conduct human evaluation on the \textit{reference} summaries.
In total, this means we conduct human evaluation on 13 sets of summaries for each dataset: six sets generated by language models adapted through few-shot prompting, four sets generated by language models adapted through zero-shot prompting (just instructions), two sets generated by state-of-the-art models fine-tuned for the respective datasets, and the official human-authored reference summaries. 

\paragraph{Annotation guidelines.}
We ask the annotators to evaluate each summary for three aspects: \textit{faithfulness}, \textit{coherence}, and \textit{relevance}, following the guidelines of \citet{fabbri-etal-2021-summeval}.\footnote{We omit evaluating fluency because we find language model outputs are mostly fluent.}
We define a summary to be faithful if ``all the information expressed by the summary can be inferred from the article'' and solicit binary decisions from the annotators.
We define a summary to be relevant if the summary ``includes only important information from the source document'' and coherent if the summary ``organizes the relevant information into a well-structured summary''.
For relevance and coherence, we ask the annotators to annotate on a 1--5 Likert scale.

We recruit annotators from Amazon Mechanical Turk, compensating them at California minimum wage of \$15.00/hr using conservative estimates of annotation time, consistent with best-practices for crowd-sourcing labor \citep{whiting2019fair}.\footnote{We estimated the time it would take workers by performing the task ourselves (it took on average 1 minute per HIT). We added a buffer of $25\%$, which would result in $31$ cents per HIT at the minimum wage (we rounded it up to $35$ cents).}
Each model summary was evaluated by three annotators; we report results based on their average score for each summary for brevity.\footnote{All underlying annotations will be made available to facilitate future analysis.}

\input{tables/human_evaluation/summarization.table}

\paragraph{Results and discussion.}
\reftab{summarization-human-evaluation} displays the results of our human evaluation for summarization.
First and foremost, we highlight the surprisingly striking finding that the reference summaries are \textbf{low quality}.
In terms of faithfulness, the reference summaries are worse than all other models on \xsum and only outperform the zero-shot non-(instruction-tuned) models on \cnndm. 
In fact, overall we observe that models with greater supervision are less faithful: zero-shot models > few-shot models > finetuned models.

Second, we highlight the importance of instruction-tuning for strong summarization performance.
Consistent with the concurrent work of \citet{goyal2022news}, we observe that zero-shot instruction-tuned models achieve the best summarization accuracy.
However, by evaluating models that both use and don't use instruction tuning, we clarify that instruction tuning is crucial: \gptdavinci performs much worse in terms of all three aspects when compared to \instructdavinci.
Looking into the model behavior, we find that the vanilla GPT-3 models often fail to follow the task instruction, frequently leading to  generations that are either exact repetitions of the source article or irrelevant to the source article.

Third, when we compare the results of human evaluations to automated evaluations, we find the two are \textit{anti-correlated}.
\texttt{ROUGE-2} scores favor fine-tuned models, whereas human judgments consistently prefer few-shot or zero-shot language models. Similarly, we find that automated faithfulness metrics are not reliable for measuring faithfulness of few-shot and zero-shot models. 
For instance, on \xsum, few-shot and zero-shot models score similarly according to automated faithfulness metrics, whereas humans overwhelmingly rate zero-shot models as more faithful.


Put together, our human evaluation presents a worrying state of affairs for summarization in the age of modern language models, especially when using \cnndm and \xsum. 
While these two datasets have served as mainstays in summarization evaluation, often functioning as the standard representatives of summarization in most contexts, we believe they will hold back and, worse, mislead progress in summarization.
We actively encourage the development of high quality summarization evaluation data, and the adoption of such data as mainstream, along with future studies on the quality of summarization metrics as well as the quality of in-context learning and other few-shot methodologies in comparison to fine-tuning.

==> tables/components/harms_bias.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
& \multicolumn{4}{c}{Copyright} & \multicolumn{4}{c}{Disinformation (reiteration)} & \multicolumn{4}{c}{BOLD (Bias in Open-Ended Language Generation Dataset)}\\
Adapter & Stereotypes (Race) & Stereotypes (Gender) & Representation (Race) & Representation (Gender) & Stereotypes (Race) & Stereotypes (Gender) & Representation (Race) & Representation (Gender) &  (Stereotypes (Race)) &Stereotypes (Gender) & Representation (Race) & Representation (Gender) \\
\midrule
Jurassic Jumbo (178B) & 0.659 & 0.37 & 0.515 & 0.224 & 0.333 & 0.5 & 0.5 & 0.5 & 0.63 & 0.438 & 0.467 & 0.172 \\
Jurassic Grande (17B) & 0.621 & 0.465 & 0.499 & 0.116 & 0.667 & 0.5 & 0.583 & 0.179 & 0.667 & 0.409 & 0.504 & 0.186 \\
Jurassic Large (7.5B) & 0.631 & 0.451 & 0.334 & 0.234 & 0.667 & 0.5 & 0.5 & 0.278 & 0.667 & 0.444 & 0.444 & 0.177 \\
Anthropic-LM (52B) & 0.665 & 0.368 & 0.502 & 0.232 & 0.667 & 0.5 & 0.5 & 0.014 & 0.641 & 0.397 & 0.382 & 0.125 \\
BLOOM (176B) & 0.667 & 0.411 & 0.382 & 0.087 & 0.667 & 0.5 & 0.604 & 0.407 & 0.667 & 0.41 & 0.3 & 0.211 \\
T0++ (11B) & 0.667 & 0.428 & 0.507 & 0.13 & 0.667 & 0.438 & 0.481 & 0.496 & 0.639 & 0.433 & 0.394 & 0.211 \\
Cohere xlarge & 0.667 & 0.365 & 0.328 & 0.221 &  & 0.5 &  & 0.5 & 0.667 & 0.436 & 0.547 & 0.179 \\
Cohere large & 0.667 & 0.421 & 0.333 & 0.224 &  &  &  &  & 0.667 & 0.415 & 0.513 & 0.2 \\
Cohere medium & 0.667 & 0.457 & 0.452 & 0.226 &  &  &  &  & 0.635 & 0.423 & 0.333 & 0.201 \\
Cohere small & 0.667 & 0.492 & 0.5 & 0.279 &  &  &  &  & 0.667 & 0.428 & 0.333 & 0.186 \\
GPT-J (6B) & 0.667 & 0.437 & 0.333 & 0.194 & 0.667 & 0.5 & 0.5 & 0.35 & 0.611 & 0.426 & 0.454 & 0.199 \\
GPT-NeoX (20B) & 0.667 & 0.441 & 0.376 & 0.216 & 0.667 & 0.333 & 0.667 & 0.378 & 0.625 & 0.419 & 0.473 & 0.163 \\
T5 (11B) & 0.667 & 0.477 & 0.333 & 0.303 & 0.667 & 0.5 & 0.333 & 0.357 &  &  & 0.667 & 0.25 \\
UL2 (20B) & 0.667 & 0.445 & 0.521 & 0.192 & 0.667 & 0.438 & 0.5 & 0.274 & 0.667 & 0.404 & 0.494 & 0.229 \\
OPT (66B) & 0.667 & 0.452 & 0.333 & 0.227 & 0.667 & 0.5 & 0.5 & 0.229 & 0.667 & 0.43 & 0.385 & 0.199 \\
OPT (175B) & 0.661 & 0.435 & 0.563 & 0.226 & 0.667 & 0.5 & 0.524 & 0.222 & 0.5 & 0.423 & 0.341 & 0.21 \\
GPT-3 (175B) & 0.667 & 0.345 & 0.584 & 0.232 &  & 0.417 & 0.667 & 0.25 & 0.667 & 0.44 & 0.431 & 0.162 \\
GPT-3 (6.7B) & 0.667 & 0.384 & 0.33 & 0.129 &  & 0.5 & 0.667 & 0.4 & 0.667 & 0.452 & 0.329 & 0.199 \\
GPT-3 (1.3B) & 0.667 & 0.461 & 0.494 & 0.226 &  &  & 0.333 & 0.375 & 0.667 & 0.448 & 0.46 & 0.181 \\
GPT-3 (350M) & 0.667 & 0.472 & 0.407 & 0.141 & 0.667 & 0.5 & 0.667 & 0.337 & 0.667 & 0.415 & 0.333 & 0.146 \\
Davinci Instruct v2 & 0.657 & 0.38 & 0.542 & 0.195 & 0.667 & 0.5 & 0.667 & 0.223 & 0.667 & 0.408 & 0.477 & 0.191 \\
Curie Instruct & 0.66 & 0.391 & 0.494 & 0.123 &  &  &  & 0.375 & 0.594 & 0.447 & 0.376 & 0.216 \\
Babbage Instruct & 0.667 & 0.424 & 0.333 & 0.159 &  & 0.5 &  & 0.5 & 0.651 & 0.424 & 0.346 & 0.174 \\
Ada Instruct & 0.524 & 0.45 & 0.457 & 0.228 &  & 0.5 & 0.667 & 0.388 & 0.667 & 0.439 & 0.394 & 0.132 \\
Davinci Codex (4000 max tokens) &  &  & 0.654 &  &  &  &  &  &  &  &  &  \\
Cushman Codex (2048 max tokens) &  &  & 0.5 & 0.5 &  &  &  &  &  &  &  &  \\
GLM (130B) & 0.667 & 0.383 & 0.433 & 0.222 & 0.586 & 0.454 & 0.5 & 0.192 & 0.639 & 0.426 & 0.41 & 0.202 \\
YaLM (100B) & 0.667 & 0.346 & 0.5 & 0.249 & 0.667 & 0.5 & 0.333 & 0.14 & 0.625 & 0.435 & 0.351 & 0.181 \\
\bottomrule
\end{tabular}}
\caption{Results for bias (harms)}
\label{fig:bias (harms)}
\end{table*}

==> tables/components/harms_copyright_metrics.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lrr}
\toprule
Adapter & Copyright (LCS) & Copyright (Edit dist.) \\
\midrule
Jurassic Jumbo (178B) & 0.007 & 8.13 \\
Jurassic Grande (17B) & 0.003 & 7.833 \\
Jurassic Large (7.5B) & 0.003 & 8.188 \\
Anthropic-LM (52B) & 0.088 & 6.495 \\
BLOOM (176B) & 0.005 & 6.974 \\
T0++ (11B) & 0.0003183909723235566 & 1.324 \\
Cohere xlarge & 0.009 & 6.736 \\
Cohere large & 0.005 & 6.708 \\
Cohere medium & 0.005 & 6.769 \\
Cohere small & 0.004 & 6.487 \\
GPT-J (6B) & 0.005 & 6.637 \\
GPT-NeoX (20B) & 0.007 & 6.766 \\
T5 (11B) & 0.006 & 1.367 \\
UL2 (20B) & 0.005 & 2.687 \\
OPT (66B) & 0.005 & 6.828 \\
OPT (175B) & 0.006 & 6.77 \\
GPT-3 (175B) & 0.071 & 6.523 \\
GPT-3 (6.7B) & 0.007 & 6.779 \\
GPT-3 (1.3B) & 0.005 & 6.861 \\
GPT-3 (350M) & 0.004 & 6.894 \\
Davinci Instruct v2 & 0.053 & 5.388 \\
Curie Instruct & 0.005 & 2.548 \\
Babbage Instruct & 0.004 & 2.191 \\
Ada Instruct & 0.004 & 1.541 \\
Davinci Codex (4000 max tokens) & 0.163 & 23.921 \\
Cushman Codex (2048 max tokens) & 0.14 & 23.679 \\
GLM (130B) & 0.005 & 6.549 \\
YaLM (100B) & 0.005 & 6.535 \\
\bottomrule
\end{tabular}}
\caption{Results for copyright metrics (harms)}
\label{fig:copyright_metrics (harms)}
\end{table}

==> tables/components/harms_disinformation_metrics.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lrr}
\toprule
Adapter & Disinformation (reiteration) (Self-BLEU) & Disinformation (reiteration) (Entropy) \\
\midrule
Jurassic Jumbo (178B) & 5.84 & 32.957 \\
Jurassic Grande (17B) & 6.23 & 34.372 \\
Jurassic Large (7.5B) & 6.41 & 36.315 \\
Anthropic-LM (52B) & 9.035 &  \\
BLOOM (176B) & 6.797 & 71.722 \\
T0++ (11B) & 43.551 & 67.022 \\
Cohere xlarge & 99.888 & 18.35 \\
Cohere large & 99.896 & 17.277 \\
Cohere medium & 100.0 & 16.843 \\
Cohere small & 100.0 & 17.637 \\
GPT-J (6B) & 4.942 & 144.273 \\
GPT-NeoX (20B) & 6.223 & 142.272 \\
T5 (11B) & 61.597 & 105.5 \\
UL2 (20B) & 20.452 & 101.787 \\
OPT (66B) & 5.761 & 122.962 \\
OPT (175B) & 6.851 & 64.903 \\
GPT-3 (175B) & 7.119 & 32.934 \\
GPT-3 (6.7B) & 6.377 & 40.444 \\
GPT-3 (1.3B) & 7.261 & 38.611 \\
GPT-3 (350M) & 6.369 & 46.338 \\
Davinci Instruct v2 & 17.379 & 12.554 \\
Curie Instruct & 14.443 & 19.369 \\
Babbage Instruct & 17.446 & 19.558 \\
Ada Instruct & 16.336 & 23.305 \\
Davinci Codex (4000 max tokens) &  &  \\
Cushman Codex (2048 max tokens) &  &  \\
GLM (130B) & 11.926 & 140.757 \\
YaLM (100B) & 7.411 & 83.826 \\
\bottomrule
\end{tabular}}
\caption{Results for disinformation metrics (harms)}
\label{fig:disinformation_metrics (harms)}
\end{table}

==> tables/components/harms_toxicity.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lrrr}
\toprule
Adapter & Copyright & Disinformation (reiteration)  & BOLD  \\
\midrule
Jurassic Jumbo (178B) & 0.029 & 0.016 & 0.002 \\
Jurassic Grande (17B) & 0.005 & 0.018 & 0.003 \\
Jurassic Large (7.5B) & 0.008 & 0.007 & 0.001 \\
Anthropic-LM (52B) & 0.01 & 0.003 & 0.004 \\
BLOOM (176B) & 0.005 & 0.003 & 0.002 \\
T0++ (11B) & 0.059 & 0.022 & 0.005 \\
Cohere xlarge & 0.03 & 0.003 &  \\
Cohere large & 0.008 & 0.003 & 0.001 \\
Cohere medium & 0.006 &  &  \\
Cohere small & 0.008 &  & 0.002 \\
GPT-J (6B) & 0.033 & 0.01 & 0.003 \\
GPT-NeoX (20B) & 0.007 & 0.017 & 0.002 \\
T5 (11B) & 0.004 & 0.012 &  \\
UL2 (20B) & 0.007 & 0.01 & 0.002 \\
OPT (66B) & 0.009 & 0.012 & 0.018 \\
OPT (175B) & 0.011 & 0.01 & 0.009 \\
GPT-3 (175B) & 0.01 &  & 0.001 \\
GPT-3 (6.7B) & 0.007 & 0.01 & 0.001 \\
GPT-3 (1.3B) & 0.008 & 0.013 & 0.002 \\
GPT-3 (350M) & 0.011 & 0.006 & 0.002 \\
Davinci Instruct v2 & 0.01 & 0.016 & 0.001 \\
Curie Instruct & 0.007 & 0.006 & 0.001 \\
Babbage Instruct & 0.007 & 0.003 & 0.003 \\
Ada Instruct & 0.008 & 0.003 & 0.002 \\
Davinci Codex (4000 max tokens) &  &  &  \\
Cushman Codex (2048 max tokens) & 0.001 &  &  \\
GLM (130B) & 0.007 & 0.012 & 0.006 \\
YaLM (100B) & 0.007 & 0.015 & 0.001 \\
\bottomrule
\end{tabular}}
\caption{Results for toxicity (harms) (toxic fraction)}
\label{fig:toxicity (harms)}
\end{table}

==> tables/components/knowledge_accuracy.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
Adapter & NaturalQ (closed-book) (F1) & HellaSwag (EM) & OpenbookQA (EM) & TruthfulQA (EM) & MMLU  (EM) & WikiFact (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.288 & 0.765 & 0.534 & 0.177 & 0.256 & 0.282 \\
Jurassic Grande (17B) & 0.226 & 0.739 & 0.52 & 0.173 & 0.276 & 0.263 \\
Jurassic Large (7.5B) & 0.197 & 0.7 & 0.514 & 0.19 & 0.265 & 0.229 \\
Anthropic-LM (52B) & 0.28 &  &  & 0.375 & 0.502 & 0.222 \\
BLOOM (176B) & 0.227 & 0.744 & 0.532 & 0.199 & 0.281 & 0.212 \\
T0++ (11B) & 0.096 &  &  & 0.336 & 0.413 & 0.107 \\
Cohere xlarge & 0.299 & 0.81 & 0.55 & 0.196 & 0.341 & 0.337 \\
Cohere large & 0.227 & 0.736 & 0.542 & 0.211 & 0.309 & 0.283 \\
Cohere medium & 0.176 & 0.706 & 0.496 & 0.185 & 0.307 & 0.248 \\
Cohere small & 0.074 & 0.483 & 0.348 & 0.185 & 0.247 & 0.15 \\
GPT-J (6B) & 0.165 & 0.663 & 0.512 & 0.191 & 0.267 & 0.166 \\
GPT-NeoX (20B) & 0.2 & 0.718 & 0.53 & 0.193 & 0.273 & 0.203 \\
T5 (11B) & 0.189 &  &  & 0.179 & 0.295 & 0.118 \\
UL2 (20B) & 0.17 &  &  & 0.199 & 0.241 & 0.159 \\
OPT (66B) & 0.26 & 0.745 & 0.534 & 0.219 & 0.258 & 0.205 \\
OPT (175B) & 0.291 & 0.791 & 0.586 & 0.248 & 0.32 & 0.214 \\
GPT-3 (175B) & 0.334 & 0.775 & 0.586 & 0.2 & 0.42 & 0.265 \\
GPT-3 (6.7B) & 0.207 & 0.682 & 0.502 & 0.237 & 0.242 & 0.192 \\
GPT-3 (1.3B) & 0.117 & 0.555 & 0.438 & 0.187 & 0.219 & 0.141 \\
GPT-3 (350M) & 0.086 & 0.435 & 0.38 & 0.22 & 0.256 & 0.085 \\
Davinci Instruct v2 & 0.388 & 0.815 & 0.594 & 0.633 & 0.574 & 0.345 \\
Curie Instruct & 0.169 & 0.676 & 0.514 & 0.202 & 0.259 & 0.169 \\
Babbage Instruct & 0.076 & 0.561 & 0.452 & 0.203 & 0.229 & 0.118 \\
Ada Instruct & 0.016 & 0.429 & 0.346 & 0.196 & 0.25 & 0.101 \\
GLM (130B) & 0.153 &  &  & 0.209 & 0.321 & 0.2 \\
YaLM (100B) & 0.14 &  &  & 0.229 & 0.267 & 0.141 \\
\bottomrule
\end{tabular}}
\caption{Results for accuracy (knowledge)}
\label{fig:accuracy (knowledge)}
\end{table*}

==> tables/components/language_accuracy.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
Adapter & The Pile (BPB) & TwitterAAE (BPB) & ICE  (BPB) & BLiMP (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.545 & 2.18 & 0.855 & 0.811 \\
Jurassic Grande (17B) & 0.601 & 2.205 & 0.874 & 0.803 \\
Jurassic Large (7.5B) & 0.646 & 2.245 & 0.901 & 0.806 \\
BLOOM (176B) & 0.569 & 1.861 & 0.715 & 0.819 \\
Cohere xlarge & 0.757 & 2.305 & 0.875 & 0.83 \\
Cohere large & 0.811 & 2.324 & 0.916 & 0.834 \\
Cohere medium & 0.845 & 2.341 & 0.954 & 0.823 \\
Cohere small & 0.996 & 2.525 & 1.112 & 0.793 \\
GPT-J (6B) & 0.49 & 1.989 & 0.752 & 0.834 \\
GPT-NeoX (20B) & 0.466 & 1.943 & 0.742 & 0.839 \\
OPT (66B) & 0.616 & 1.723 & 0.763 & 0.827 \\
OPT (175B) & 0.591 & 1.73 & 0.74 & 0.831 \\
GPT-3 (175B) & 0.713 & 2.141 & 0.977 & 0.84 \\
GPT-3 (6.7B) & 0.789 & 2.21 & 0.958 & 0.832 \\
GPT-3 (1.3B) & 0.866 & 2.291 & 1.048 & 0.833 \\
GPT-3 (350M) & 0.96 & 2.395 & 1.136 & 0.818 \\
Davinci Instruct v2 & 0.578 & 2.147 & 0.823 & 0.812 \\
Curie Instruct & 0.969 & 2.628 & 1.192 & 0.76 \\
Babbage Instruct & 1.103 & 2.946 & 1.326 & 0.769 \\
Ada Instruct & 1.61 & 3.505 & 1.975 & 0.728 \\
\bottomrule
\end{tabular}}
\caption{Results for accuracy (language)}
\label{fig:accuracy (language)}
\end{table*}

==> tables/components/reasoning_accuracy.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
Adapter & Synthetic reasoning (abstract symbols) (EM) & Synthetic reasoning (natural language) (F1) & bAbI (EM) & Dyck (EM) & GSM8K (EM) & MATH (Equivalent) & MATH (chain-of-thoughts) (Equivalent) & HumanEval (Code) (pass@1) & LSAT (EM) & LegalSupport (EM) & Data imputation (EM) & Entity matching (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.227 & 0.163 & 0.353 & 0.442 & 0.042 & 0.082 & 0.011 &  & 0.213 & 0.468 & 0.735 & 0.849 \\
Jurassic Grande (17B) & 0.207 & 0.167 & 0.336 & 0.708 & 0.051 & 0.092 & 0.009 &  & 0.187 & 0.536 & 0.753 & 0.824 \\
Jurassic Large (7.5B) & 0.16 & 0.157 & 0.322 & 0.456 & 0.021 & 0.048 & 0.002 &  & 0.2 & 0.515 & 0.725 & 0.824 \\
Anthropic-LM (52B) & 0.44 & 0.377 & 0.37 & 0.81 & 0.156 & 0.167 & 0.158 &  & 0.2 & 0.613 & 0.729 & 0.571 \\
BLOOM (176B) & 0.3 & 0.173 & 0.286 & 0.51 & 0.091 & 0.041 & 0.057 &  & 0.196 & 0.534 & 0.702 & 0.829 \\
T0++ (11B) & 0.013 & 0.04 & 0.099 & 0.026 &  &  &  &  & 0.191 & 0.599 & 0.22 & 0.843 \\
Cohere xlarge & 0.107 &  & 0.294 & 0.558 & 0.102 & 0.14 & 0.048 &  & 0.183 & 0.515 & 0.83 & 0.824 \\
Cohere large & 0.107 &  & 0.212 & 0.486 & 0.031 & 0.066 & 0.007 &  & 0.191 & 0.511 & 0.735 & 0.614 \\
Cohere medium & 0.08 &  & 0.265 & 0.512 & 0.014 & 0.048 & 0.023 &  & 0.2 & 0.53 & 0.721 & 0.176 \\
Cohere small & 0.08 &  & 0.165 & 0.378 & 0.004 & 0.023 & 0.002 &  & 0.165 & 0.485 & 0.458 & 0.176 \\
GPT-J (6B) & 0.107 & 0.15 & 0.32 & 0.294 & 0.034 & 0.11 & 0.025 &  & 0.152 & 0.468 & 0.658 & 0.183 \\
GPT-NeoX (20B) & 0.16 & 0.11 & 0.312 & 0.718 & 0.054 & 0.112 & 0.071 &  & 0.17 & 0.524 & 0.714 & 0.824 \\
T5 (11B) & 0.18 & 0.1 & 0.217 & 0.352 & 0.025 &  &  &  & 0.165 & 0.544 & 0.679 & 0.811 \\
UL2 (20B) & 0.187 & 0.067 & 0.23 & 0.114 & 0.029 &  &  &  & 0.191 & 0.513 & 0.731 & 0.59 \\
OPT (66B) & 0.1 & 0.183 & 0.273 & 0.474 & 0.018 & 0.043 & 0.005 &  & 0.191 & 0.519 & 0.708 & 0.669 \\
OPT (175B) & 0.16 & 0.283 & 0.262 & 0.488 & 0.046 & 0.059 & 0.007 &  & 0.2 & 0.515 & 0.721 & 0.764 \\
GPT-3 (175B) & 0.287 & 0.18 & 0.334 & 0.664 & 0.102 & 0.092 & 0.023 &  & 0.161 & 0.493 & 0.836 & 0.815 \\
GPT-3 (6.7B) & 0.167 & 0.137 & 0.262 & 0.494 & 0.02 & 0.046 & 0.016 &  & 0.178 & 0.532 & 0.807 & 0.665 \\
GPT-3 (1.3B) & 0.087 & 0.067 & 0.235 & 0.484 & 0.008 & 0.043 & 0.009 &  & 0.252 & 0.515 & 0.609 & 0.824 \\
GPT-3 (350M) & 0.087 & 0.123 & 0.234 & 0.424 & 0.008 & 0.057 & 0.002 &  & 0.196 & 0.485 & 0.58 & 0.673 \\
Davinci Instruct v2 & 0.5 & 0.627 & 0.464 & 0.594 & 0.35 & 0.33 & 0.35 &  & 0.213 & 0.601 & 0.83 & 0.923 \\
Curie Instruct & 0.167 & 0.247 & 0.239 & 0.416 & 0.002 & 0.048 & 0.007 &  & 0.174 & 0.511 & 0.784 & 0.817 \\
Babbage Instruct & 0.02 & 0.117 & 0.208 & 0.226 & 0.001 & 0.016 &  &  & 0.187 & 0.515 & 0.704 & 0.824 \\
Ada Instruct & 0.12 & 0.102 & 0.155 & 0.16 & 0.003 & 0.03 &  &  & 0.235 & 0.517 & 0.509 & 0.824 \\
Davinci Codex (4000 max tokens) & 0.553 & 0.727 & 0.456 & 0.802 & 0.521 & 0.405 & 0.476 & 0.482 &  &  &  &  \\
Cushman Codex (2048 max tokens) & 0.373 & 0.167 & 0.287 & 0.402 & 0.042 & 0.108 & 0.046 & 0.317 &  &  &  &  \\
GLM (130B) & 0.227 & 0.247 & 0.289 & 0.542 & 0.07 &  & 0.032 &  & 0.191 & 0.519 & 0.646 & 0.613 \\
YaLM (100B) & 0.04 & 0.127 & 0.213 & 0.616 & 0.021 &  &  &  & 0.178 & 0.485 & 0.427 & 0.176 \\
\bottomrule
\end{tabular}}
\caption{Results for accuracy (reasoning)}
\label{fig:accuracy (reasoning)}
\end{table*}

==> tables/human_evaluation/summarization.table.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{llrrrrrr}
\toprule
 &  & \multicolumn{3}{c}{\cnndm} & \multicolumn{3}{c}{\xsum} \\
Setting & Models & Faithfulness & Coherence & Relevance & Faithfulness & Coherence & Relevance \\
\midrule
\multirow[c]{4}{*}{Zero-shot language models} & \gptcurie & 0.29 & 1.77 & 1.93 & 0.77 & 3.16 & 3.39 \\
 & \gptdavinci & 0.76 & 2.65 & 3.50 & 0.80 & 2.78 & 3.52 \\
 & \instructcurie & 0.97 & 4.24 & 4.59 & 0.96 & 4.27 & 4.34 \\
 & \instructdavinci & 0.99 & 4.15 & 4.60 & 0.97 & 4.41 & 4.28 \\
\midrule
\multirow[c]{6}{*}{Five-shot language models} & \anthropic & 0.94 & 3.88 & 4.33 & 0.70 & 4.77 & 4.14 \\
 & \coherexl & 0.99 & 3.42 & 4.48 & 0.63 & 4.79 & 4.00 \\
 & \glm & 0.94 & 3.69 & 4.24 & 0.74 & 4.72 & 4.12 \\
 & \optonesevenfive & 0.96 & 3.64 & 4.33 & 0.67 & 4.80 & 4.01 \\
 & \gptdavinci & 0.99 & 3.95 & 4.34 & 0.69 & 4.69 & 4.03 \\
 & \instructdavinci & 0.98 & 4.13 & 4.49 & 0.77 & 4.83 & 4.33 \\
\midrule
\multirow[c]{2}{*}{Fine-tuned language models} & Brio & 0.94 & 3.94 & 4.40 & 0.58 & 4.68 & 3.89 \\
 & Pegasus & 0.97 & 3.93 & 4.38 & 0.57 & 4.73 & 3.85 \\
\midrule
Human generated & Reference summaries & 0.84 & 3.20 & 3.94 & 0.37 & 4.13 & 3.00 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Human evaluation for summarization scenarios.} 
We conduct human evaluation for 13 sets of summaries for both \cnndm and \xsum.}
\label{tab:summarization-human-evaluation}
\end{table*}

==> tables/metric-metric.table.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
  &   & Accuracy & Calibration & Robustness & Fairness & Bias & Toxicity & Efficiency \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{Pearson}} & Accuracy & \color{lightgray} 1.0 (0.0) & 0.4 (3.3e-11) & 0.93 (2.6e-109) & 0.98 (1.9e-167) & 0.28 (0.001) & 0.15 (0.042) & -0.22 (0.0068) \\
 & Calibration & \color{lightgray} 0.4 (3.3e-11) & \color{lightgray} 1.0 (0.0) & 0.41 (1e-11) & 0.42 (4.6e-12) & 0.15 (0.18) & -0.21 (0.019) & 0.019 (0.84) \\
 & Robustness & \color{lightgray} 0.93 (2.6e-109) & \color{lightgray} 0.41 (1e-11) & \color{lightgray} 1.0 (0.0) & 0.93 (3.6e-112) & 0.00038 (1.0) & -0.079 (0.37) & -0.24 (0.0074) \\
 & Fairness & \color{lightgray} 0.98 (1.9e-167) & \color{lightgray} 0.42 (4.6e-12) & \color{lightgray} 0.93 (3.6e-112) & \color{lightgray} 1.0 (0.0) & 0.067 (0.54) & -0.094 (0.28) & -0.18 (0.043) \\
 & Bias & \color{lightgray} 0.28 (0.001) & \color{lightgray} 0.15 (0.18) & \color{lightgray} 0.00038 (1.0) & \color{lightgray} 0.067 (0.54) & \color{lightgray} 1.0 (0.0) & -0.14 (0.11) & 0.18 (0.16) \\
 & Toxicity & \color{lightgray} 0.15 (0.042) & \color{lightgray} -0.21 (0.019) & \color{lightgray} -0.079 (0.37) & \color{lightgray} -0.094 (0.28) & \color{lightgray} -0.14 (0.11) & \color{lightgray} 1.0 (0.0) & 0.0024 (0.98) \\
 & Efficiency & \color{lightgray} -0.22 (0.0068) & \color{lightgray} 0.019 (0.84) & \color{lightgray} -0.24 (0.0074) & \color{lightgray} -0.18 (0.043) & \color{lightgray} 0.18 (0.16) & \color{lightgray} 0.0024 (0.98) & \color{lightgray} 1.0 (0.0) \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{Spearman}} & Accuracy & \color{lightgray} 1.0 (0.0) & 0.46 (2e-14) & 0.92 (1e-100) & 0.97 (1.8e-159) & 0.29 (0.00064) & -0.15 (0.049) & -0.24 (0.0024) \\
 & Calibration & \color{lightgray} 0.46 (2e-14) & \color{lightgray} 1.0 (0.0) & 0.49 (1.1e-16) & 0.49 (2.4e-16) & 0.05 (0.65) & -0.44 (2.3e-07) & -0.0042 (0.96) \\
 & Robustness & \color{lightgray} 0.92 (1e-100) & \color{lightgray} 0.49 (1.1e-16) & \color{lightgray} 1.0 (0.0) & 0.94 (4.1e-113) & -0.14 (0.19) & -0.36 (2.3e-05) & -0.14 (0.12) \\
 & Fairness & \color{lightgray} 0.97 (1.8e-159) & \color{lightgray} 0.49 (2.4e-16) & \color{lightgray} 0.94 (4.1e-113) & \color{lightgray} 1.0 (0.0) & -0.1 (0.36) & -0.42 (8.7e-07) & 0.051 (0.57) \\
 & Bias & \color{lightgray} 0.29 (0.00064) & \color{lightgray} 0.05 (0.65) & \color{lightgray} -0.14 (0.19) & \color{lightgray} -0.1 (0.36) & \color{lightgray} 1.0 (0.0) & -0.1 (0.25) & 0.16 (0.21) \\
 & Toxicity & \color{lightgray} -0.15 (0.049) & \color{lightgray} -0.44 (2.3e-07) & \color{lightgray} -0.36 (2.3e-05) & \color{lightgray} -0.42 (8.7e-07) & \color{lightgray} -0.1 (0.25) & \color{lightgray} 1.0 (0.0) & 0.42 (3.5e-05) \\
 & Efficiency & \color{lightgray} -0.24 (0.0024) & \color{lightgray} -0.0042 (0.96) & \color{lightgray} -0.14 (0.12) & \color{lightgray} 0.051 (0.57) & \color{lightgray} 0.16 (0.21) & \color{lightgray} 0.42 (3.5e-05) & \color{lightgray} 1.0 (0.0) \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{Kendall tau}} & Accuracy & \color{lightgray} 1.0 (4.9e-147) & 0.33 (1.6e-14) & 0.77 (5.8e-73) & 0.88 (5e-94) & 0.17 (0.0026) & -0.11 (0.041) & -0.14 (0.0091) \\
 & Calibration & \color{lightgray} 0.33 (1.6e-14) & \color{lightgray} 1.0 (0.0) & 0.35 (5e-16) & 0.35 (1.4e-16) & 0.037 (0.62) & -0.32 (6.1e-07) & -0.0039 (0.95) \\
 & Robustness & \color{lightgray} 0.77 (5.8e-73) & \color{lightgray} 0.35 (5e-16) & \color{lightgray} 1.0 (1.5e-121) & 0.79 (2.4e-77) & -0.1 (0.18) & -0.27 (2.3e-05) & -0.083 (0.17) \\
 & Fairness & \color{lightgray} 0.88 (5e-94) & \color{lightgray} 0.35 (1.4e-16) & \color{lightgray} 0.79 (2.4e-77) & \color{lightgray} 1.0 (1.4e-121) & -0.052 (0.49) & -0.31 (1.4e-06) & 0.036 (0.55) \\
 & Bias & \color{lightgray} 0.17 (0.0026) & \color{lightgray} 0.037 (0.62) & \color{lightgray} -0.1 (0.18) & \color{lightgray} -0.052 (0.49) & \color{lightgray} 1.0 (9.8e-67) & -0.073 (0.23) & 0.1 (0.22) \\
 & Toxicity & \color{lightgray} -0.11 (0.041) & \color{lightgray} -0.32 (6.1e-07) & \color{lightgray} -0.27 (2.3e-05) & \color{lightgray} -0.31 (1.4e-06) & \color{lightgray} -0.073 (0.23) & \color{lightgray} 1.0 (6.4e-68) & 0.3 (7.1e-05) \\
 & Efficiency & \color{lightgray} -0.14 (0.0091) & \color{lightgray} -0.0039 (0.95) & \color{lightgray} -0.083 (0.17) & \color{lightgray} 0.036 (0.55) & \color{lightgray} 0.1 (0.22) & \color{lightgray} 0.3 (7.1e-05) & \color{lightgray} 1.0 (1.4e-74) \\
\bottomrule
\end{tabular}}
\caption{\textbf{Relationship between metrics.} To summarize the relationship between metrics (across all models and scenarios), we report the Kendall tau correlation between pairs of metrics, with \todo{} indicating significance at \todo{}. \todo{we need to figure out how to do confidences here. Not super convinced about these results}}
\label{tab:metric-metric}
\end{table*}

==> tables/metrics/tasks_accuracy.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
Adapter & MMLU (EM) & BoolQ (EM) & NarrativeQA (F1) & NaturalQ (closed-book) (F1) & NaturalQ (open-book) (F1) & QuAC (F1) & HellaSwag (EM) & OpenbookQA (EM) & TruthfulQA (EM) & CNN/DailyMail (ROUGE-2) & XSUM (ROUGE-2) & IMDB (EM) & CivilComments (EM) & RAFT (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.256 & 0.791 & 0.688 & 0.288 &  & 0.365 & 0.765 & 0.534 & 0.177 & 0.149 & 0.122 & 0.927 & 0.407 & 0.702 \\
Jurassic Grande (17B) & 0.276 & 0.727 & 0.691 & 0.226 &  & 0.372 & 0.739 & 0.52 & 0.173 & 0.152 & 0.117 & 0.949 & 0.788 & 0.664 \\
Jurassic Large (7.5B) & 0.265 & 0.712 & 0.634 & 0.197 &  & 0.304 & 0.7 & 0.514 & 0.19 & 0.13 & 0.103 & 0.952 & 0.777 & 0.536 \\
Anthropic-LM (52B) & 0.502 & 0.829 & 0.718 & 0.28 & 0.672 & 0.449 &  &  & 0.375 & 0.155 & 0.126 & 0.93 & 0.589 & 0.68 \\
BLOOM (176B) & 0.281 & 0.745 & 0.671 & 0.227 & 0.456 & 0.358 & 0.744 & 0.532 & 0.199 & 0.113 & 0.032 & 0.944 & 0.614 & 0.584 \\
T0++ (11B) & 0.413 & 0.592 & 0.355 & 0.096 & 0.604 & 0.154 &  &  & 0.336 & 0.121 & 0.106 & 0.57 & 0.672 & 0.411 \\
Cohere xlarge & 0.341 & 0.784 & 0.647 & 0.299 & 0.394 & 0.368 & 0.81 & 0.55 & 0.196 & 0.166 & 0.128 & 0.938 & 0.389 & 0.602 \\
Cohere large & 0.309 & 0.744 & 0.641 & 0.227 & 0.472 & 0.343 & 0.736 & 0.542 & 0.211 & 0.15 & 0.102 & 0.925 & 0.277 & 0.609 \\
Cohere medium & 0.307 & 0.643 & 0.578 & 0.176 & 0.331 & 0.284 & 0.706 & 0.496 & 0.185 & 0.129 & 0.085 & 0.886 & 0.212 & 0.523 \\
Cohere small & 0.247 & 0.481 & 0.31 & 0.074 & 0.234 & 0.213 & 0.483 & 0.348 & 0.185 & 0.08 & 0.027 & 0.521 & 0.805 & 0.509 \\
GPT-J (6B) & 0.267 & 0.544 & 0.547 & 0.165 & 0.412 & 0.319 & 0.663 & 0.512 & 0.191 & 0.143 & 0.095 & 0.953 & 0.284 & 0.616 \\
GPT-NeoX (20B) & 0.273 & 0.72 & 0.605 & 0.2 & 0.446 & 0.342 & 0.718 & 0.53 & 0.193 & 0.145 & 0.095 & 0.945 & 0.224 & 0.511 \\
T5 (11B) & 0.295 & 0.831 & 0.086 & 0.189 & 0.29 & 0.119 &  &  & 0.179 & 0.054 & 0.017 & 0.382 & 0.604 & 0.336 \\
UL2 (20B) & 0.241 & 0.806 & 0.092 & 0.17 & 0.191 & 0.154 &  &  & 0.199 & 0.053 & 0.05 & 0.403 & 0.62 & 0.293 \\
OPT (66B) & 0.258 & 0.757 & 0.652 & 0.26 & 0.438 & 0.35 & 0.745 & 0.534 & 0.219 & 0.147 & 0.122 & 0.921 & 0.198 & 0.575 \\
OPT (175B) & 0.32 & 0.816 & 0.671 & 0.291 & 0.458 & 0.365 & 0.791 & 0.586 & 0.248 & 0.167 & 0.156 & 0.948 & 0.215 & 0.6 \\
GPT-3 (175B) & 0.42 & 0.734 & 0.697 & 0.334 & 0.376 & 0.355 & 0.775 & 0.586 & 0.2 & 0.148 & 0.139 & 0.913 & 0.294 & 0.655 \\
GPT-3 (6.7B) & 0.242 & 0.642 & 0.594 & 0.207 & 0.376 & 0.319 & 0.682 & 0.502 & 0.237 & 0.137 & 0.103 & 0.902 & 0.337 & 0.484 \\
GPT-3 (1.3B) & 0.219 & 0.502 & 0.516 & 0.117 & 0.307 & 0.273 & 0.555 & 0.438 & 0.187 & 0.125 & 0.02 & 0.52 & 0.646 & 0.491 \\
GPT-3 (350M) & 0.256 & 0.61 & 0.333 & 0.086 & 0.304 & 0.226 & 0.435 & 0.38 & 0.22 & 0.107 & 0.003 & 0.898 & 0.662 & 0.386 \\
Davinci Instruct v2 & 0.574 & 0.863 & 0.748 & 0.388 & 0.68 & 0.445 & 0.815 & 0.594 & 0.633 & 0.163 & 0.146 & 0.947 & 0.688 & 0.691 \\
Curie Instruct & 0.259 & 0.616 & 0.569 & 0.169 & 0.403 & 0.376 & 0.676 & 0.514 & 0.202 & 0.157 & 0.075 & 0.915 & 0.679 & 0.495 \\
Babbage Instruct & 0.229 & 0.394 & 0.429 & 0.076 & 0.33 & 0.274 & 0.561 & 0.452 & 0.203 & 0.161 & 0.047 & 0.923 & 0.809 & 0.53 \\
Ada Instruct & 0.25 & 0.509 & 0.218 & 0.016 & 0.205 & 0.177 & 0.429 & 0.346 & 0.196 & 0.134 & 0.033 & 0.839 & 0.799 & 0.423 \\
GLM (130B) & 0.321 & 0.839 & 0.739 & 0.153 & 0.163 & 0.292 &  &  & 0.209 & 0.153 & 0.136 & 0.955 & 0.81 & 0.593 \\
YaLM (100B) & 0.267 & 0.648 & 0.536 & 0.14 & 0.375 & 0.307 &  &  & 0.229 & 0.022 & 0.022 & 0.8 & 0.753 & 0.555 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Accuracy of all models across all generic scenarios.}}
\label{tab:accuracy-generic}
\end{table*}

==> tables/metrics/tasks_bias.tex <==
\begin{table*}[htp]
% \resizebox{\textwidth}{!}{
\begin{tabular}{lllll@{\hspace*{2.75em}}llll}
\toprule
& \multicolumn{4}{c@{\hspace*{2.75em}}}{CNN/DailyMail} & \multicolumn{4}{c}{XSUM} \\
& \multicolumn{2}{c}{Stereotypes} 
& \multicolumn{2}{c@{\hspace*{2.75em}}}{Representation}
& \multicolumn{2}{c}{Stereotypes}
& \multicolumn{2}{c}{Representation} \\
Adapter & Race & Gender & Race & Gender & Race & Gender & Race & Gender \\
\midrule
Jurassic Jumbo (178B) & 0.608 & 0.383 & 0.289 & 0.12 & 0.667 & 0.453 & 0.532 & 0.205 \\
Jurassic Grande (17B) & 0.639 & 0.4 & 0.386 & 0.145 & 0.667 & 0.432 & 0.545 & 0.158 \\
Jurassic Large (7.5B) & 0.608 & 0.381 & 0.29 & 0.164 & 0.667 & 0.449 & 0.455 & 0.14 \\
Anthropic-LM (52B) & 0.658 & 0.418 & 0.278 & 0.09 & 0.667 & 0.476 & 0.467 & 0.238 \\
BLOOM (176B) & 0.647 & 0.399 & 0.403 & 0.1 & 0.667 & 0.5 & 0.333 & 0.222 \\
T0++ (11B) & 0.635 & 0.398 & 0.293 & 0.099 & 0.667 & 0.44 & 0.441 & 0.229 \\
Cohere xlarge & 0.603 & 0.387 & 0.34 & 0.118 & 0.667 & 0.468 & 0.667 & 0.18 \\
Cohere large & 0.613 & 0.398 & 0.306 & 0.128 & 0.667 & 0.438 & 0.667 & 0.142 \\
Cohere medium & 0.667 & 0.38 & 0.356 & 0.119 & 0.667 & 0.468 & 0.605 & 0.168 \\
Cohere small & 0.608 & 0.351 & 0.164 & 0.16 & 0.667 & 0.386 & 0.667 & 0.181 \\
GPT-J (6B) & 0.657 & 0.396 & 0.428 & 0.158 & 0.667 & 0.467 & 0.509 & 0.163 \\
GPT-NeoX (20B) & 0.62 & 0.399 & 0.339 & 0.139 & 0.667 & 0.443 & 0.467 & 0.154 \\
T5 (11B) & 0.667 & 0.368 & 0.398 & 0.09 & 0.667 & 0.5 & 0.333 & 0.228 \\
UL2 (20B) & 0.667 & 0.421 & 0.429 & 0.165 & 0.667 & 0.399 & 0.504 & 0.247 \\
OPT (66B) & 0.609 & 0.38 & 0.338 & 0.158 & 0.583 & 0.462 & 0.447 & 0.193 \\
OPT (175B) & 0.609 & 0.402 & 0.344 & 0.129 & 0.667 & 0.431 & 0.362 & 0.191 \\
GPT-3 (175B) & 0.652 & 0.406 & 0.27 & 0.15 & 0.667 & 0.493 & 0.515 & 0.205 \\
GPT-3 (6.7B) & 0.618 & 0.381 & 0.265 & 0.15 & 0.667 & 0.435 & 0.667 & 0.179 \\
GPT-3 (1.3B) & 0.646 & 0.377 & 0.407 & 0.123 & 0.667 & 0.429 & 0.515 & 0.158 \\
GPT-3 (350M) & 0.639 & 0.385 & 0.238 & 0.146 &  & 0.5 & 0.667 & 0.079 \\
Davinci Instruct v2 & 0.62 & 0.392 & 0.294 & 0.119 & 0.667 & 0.456 & 0.545 & 0.217 \\
Curie Instruct & 0.64 & 0.379 & 0.327 & 0.144 & 0.667 & 0.454 & 0.561 & 0.197 \\
Babbage Instruct & 0.595 & 0.377 & 0.301 & 0.13 & 0.667 & 0.41 & 0.48 & 0.165 \\
Ada Instruct & 0.644 & 0.363 & 0.315 & 0.129 & 0.667 & 0.5 & 0.619 & 0.154 \\
GLM (130B) & 0.61 & 0.385 & 0.318 & 0.131 & 0.667 & 0.447 & 0.579 & 0.203 \\
YaLM (100B) & 0.667 & 0.377 & 0.667 & 0.19 & 0.667 & 0.443 & 0.667 & 0.159 \\
\bottomrule
\end{tabular}%}
\caption{\textbf{Bias in model generations for all models across all generic scenarios, referring to both gender and racial demographic representation and stereotypical associations.}}
\label{tab:bias-generic}
\end{table*}

==> tables/metrics/tasks_calibration.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
Adapter & MMLU & BoolQ & NarrativeQA & NaturalQ (closed-book) & NaturalQ (open-book)& QuAC & HellaSwag & OpenbookQA & TruthfulQA  & IMDB & CivilComments  & RAFT \\
\midrule
Jurassic Jumbo (178B) & 0.118 & 0.207 & 0.033 & 0.036 &  & 0.032 & 0.217 & 0.25 & 0.116 & 0.073 & 0.586 & 0.223 \\
Jurassic Grande (17B) & 0.115 & 0.271 & 0.045 & 0.024 &  & 0.026 & 0.213 & 0.258 & 0.116 & 0.051 & 0.21 & 0.199 \\
Jurassic Large (7.5B) & 0.144 & 0.287 & 0.042 & 0.014 &  & 0.02 & 0.192 & 0.25 & 0.121 & 0.048 & 0.219 & 0.316 \\
Anthropic-LM (52B) & 0.502 & 0.171 & 0.704 & 0.84 & 0.537 & 0.815 &  &  & 0.625 & 0.07 & 0.411 & 0.323 \\
BLOOM (176B) & 0.13 & 0.244 & 0.281 & 0.113 & 0.237 & 0.107 & 0.293 & 0.25 & 0.112 & 0.294 & 0.194 & 0.48 \\
T0++ (11B) & 0.162 & 0.39 & 0.101 & 0.023 & 0.318 & 0.008 &  &  & 0.163 & 0.084 & 0.331 & 0.336 \\
Cohere xlarge & 0.144 & 0.092 & 0.07 & 0.071 & 0.123 & 0.069 & 0.34 & 0.235 & 0.119 & 0.071 & 0.235 & 0.29 \\
Cohere large & 0.124 & 0.125 & 0.036 & 0.011 & 0.241 & 0.023 & 0.288 & 0.225 & 0.088 & 0.087 & 0.317 & 0.244 \\
Cohere medium & 0.118 & 0.132 & 0.054 & 0.023 & 0.158 & 0.048 & 0.271 & 0.275 & 0.097 & 0.11 & 0.363 & 0.261 \\
Cohere small & 0.148 & 0.142 & 0.046 & 0.039 & 0.179 & 0.038 & 0.083 & 0.379 & 0.11 & 0.087 & 0.15 & 0.218 \\
GPT-J (6B) & 0.131 & 0.077 & 0.219 & 0.079 & 0.187 & 0.105 & 0.233 & 0.237 & 0.073 & 0.285 & 0.199 & 0.616 \\
GPT-NeoX (20B) & 0.108 & 0.225 & 0.253 & 0.108 & 0.213 & 0.121 & 0.278 & 0.23 & 0.093 & 0.22 & 0.287 & 0.511 \\
T5 (11B) & 0.117 & 0.473 & 8.25e-11 & 0.071 & 0.001 & 2.04e-09 &  &  & 0.054 & 0.278 & 0.228 & 0.334 \\
UL2 (20B) & 0.188 & 0.323 & 2.0e-05 & 0.081 & 1.0e-06 & 0.001 &  &  & 0.177 & 0.255 & 0.159 & 0.29 \\
OPT (66B) & 0.136 & 0.188 & 0.273 & 0.149 & 0.223 & 0.109 & 0.293 & 0.237 & 0.099 & 0.325 & 0.405 & 0.575 \\
OPT (175B) & 0.131 & 0.234 & 0.27 & 0.164 & 0.255 & 0.135 & 0.325 & 0.209 & 0.043 & 0.21 & 0.334 & 0.359 \\
GPT-3 (175B) & 0.111 & 0.164 & 0.205 & 0.143 & 0.143 & 0.068 & 0.31 & 0.204 & 0.201 & 0.16 & 0.258 & 0.449 \\
GPT-3 (6.7B) & 0.146 & 0.159 & 0.17 & 0.096 & 0.148 & 0.036 & 0.25 & 0.26 & 0.05 & 0.273 & 0.197 & 0.399 \\
GPT-3 (1.3B) & 0.147 & 0.137 & 0.171 & 0.045 & 0.099 & 0.036 & 0.144 & 0.3 & 0.153 & 0.267 & 0.237 & 0.411 \\
GPT-3 (350M) & 0.142 & 0.228 & 0.106 & 0.027 & 0.101 & 0.033 & 0.057 & 0.346 & 0.084 & 0.333 & 0.198 & 0.335 \\
Davinci Instruct v2 & 0.182 & 0.764 & 0.312 & 0.233 & 0.391 & 0.197 & 0.286 & 0.238 & 0.231 & 0.9 & 0.629 & 0.641 \\
Curie Instruct & 0.399 & 0.615 & 0.182 & 0.091 & 0.141 & 0.15 & 0.153 & 0.321 & 0.35 & 0.914 & 0.678 & 0.495 \\
Babbage Instruct & 0.323 & 0.223 & 0.168 & 0.061 & 0.135 & 0.091 & 0.083 & 0.362 & 0.255 & 0.922 & 0.807 & 0.525 \\
Ada Instruct & 0.518 & 0.436 & 0.056 & 0.124 & 0.13 & 0.05 & 0.103 & 0.487 & 0.481 & 0.722 & 0.787 & 0.389 \\
GLM (130B) & 0.125 & 0.236 & 0.297 & 0.077 & 0.001 & 0.076 &  &  & 0.104 & 0.216 & 0.14 & 0.351 \\
YaLM (100B) & 0.127 & 0.173 & 0.239 & 0.063 & 0.173 & 0.101 &  &  & 0.081 & 0.504 & 0.173 & 0.352 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Calibration error (ECE 10-bin) for all models across all generic scenarios.}}
\label{tab:calibration-generic}
\end{table*}

==> tables/metrics/tasks_efficiency.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
Adapter & MMLU  & BoolQ  & NarrativeQA & NaturalQ (closed-book) & NaturalQ (open-book) & QuAC & HellaSwag & OpenbookQA  & TruthfulQA  & CNN/DailyMail  & XSUM  & IMDB  & CivilComments  & RAFT  \\
\midrule
Jurassic Jumbo (178B) & 0.457 & 0.728 & 1.124 & 0.475 &  & 1.835 & 0.284 & 0.259 & 0.453 & 4.12 & 1.586 & 0.774 & 0.564 & 0.693 \\
Jurassic Grande (17B) & 0.411 & 0.625 & 0.916 & 0.483 &  & 1.33 & 0.33 & 0.281 & 0.403 & 2.231 & 1.035 & 0.673 & 0.499 & 0.6 \\
Jurassic Large (7.5B) & 0.377 & 0.567 & 0.791 & 0.378 &  & 1.035 & 0.253 & 0.238 & 0.372 & 2.11 & 0.882 & 0.582 & 0.444 & 0.504 \\
Anthropic-LM (52B) & 0.578 & 0.75 & 1.838 & 0.778 & 2.228 & 3.397 &  &  & 0.593 & 4.298 & 2.342 & 0.886 & 0.612 & 0.877 \\
BLOOM (176B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
T0++ (11B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Cohere xlarge &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Cohere large & 0.317 & 0.505 & 0.675 & 0.338 & 0.692 & 1.174 & 0.225 & 0.201 & 0.324 & 2.651 & 1.031 & 0.619 & 0.386 & 0.458 \\
Cohere medium & 0.281 & 0.402 & 0.51 & 0.259 & 0.598 & 0.716 & 0.204 & 0.187 & 0.287 & 1.328 & 0.689 & 0.483 & 0.328 & 0.367 \\
Cohere small & 0.284 & 0.436 & 0.526 & 0.259 & 0.436 & 0.602 & 0.223 & 0.214 & 0.288 & 1.041 & 0.602 & 0.52 & 0.338 & 0.372 \\
GPT-J (6B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
GPT-NeoX (20B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
T5 (11B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
UL2 (20B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
OPT (66B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
OPT (175B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
GPT-3 (175B) & 0.212 & 0.337 & 0.522 & 0.516 & 1.15 & 1.078 & 0.193 & 0.184 & 0.216 & 2.44 & 1.097 & 0.351 & 0.332 & 0.434 \\
GPT-3 (6.7B) & 0.092 & 0.132 & 0.186 & 0.16 & 0.405 & 0.358 & 0.084 & 0.079 & 0.094 & 0.763 & 0.298 & 0.142 & 0.126 & 0.152 \\
GPT-3 (1.3B) & 0.119 & 0.149 & 0.198 & 0.183 & 0.51 & 0.294 & 0.113 & 0.111 & 0.12 & 0.721 & 0.238 & 0.154 & 0.145 & 0.169 \\
GPT-3 (350M) & 0.14 & 0.165 & 0.249 & 0.195 & 0.469 & 0.31 & 0.138 & 0.136 & 0.141 & 0.644 & 0.198 & 0.167 & 0.165 & 0.187 \\
Davinci Instruct v2 & 0.196 & 0.332 & 0.608 & 0.429 & 0.635 & 1.038 & 0.171 & 0.158 & 0.202 & 2.53 & 1.112 & 0.358 & 0.307 & 0.425 \\
Curie Instruct & 0.133 & 0.17 & 0.242 & 0.192 & 0.299 & 0.323 & 0.125 & 0.119 & 0.134 & 0.876 & 0.371 & 0.179 & 0.169 & 0.189 \\
Babbage Instruct & 0.133 & 0.178 & 0.289 & 0.18 & 0.284 & 0.348 & 0.125 & 0.122 & 0.134 & 1.012 & 0.414 & 0.19 & 0.167 & 0.192 \\
Ada Instruct & 0.088 & 0.127 & 0.201 & 0.124 & 0.216 & 0.263 & 0.079 & 0.076 & 0.089 & 0.741 & 0.315 & 0.137 & 0.117 & 0.14 \\
GLM (130B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
YaLM (100B) &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}}
\caption{\textbf{Idealized denoised runtime in seconds for all models across all generic scenarios.}}
\label{tab:efficiency-generic}
\end{table*}

==> tables/metrics/tasks_fairness.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
Adapter & MMLU (EM) & BoolQ (EM) & NarrativeQA (F1) & NaturalQ (closed-book) (F1) & NaturalQ (open-book) (F1) & QuAC (F1) & HellaSwag (EM) & OpenbookQA (EM) & TruthfulQA (EM) & IMDB (EM) & CivilComments (EM) & RAFT (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.234 & 0.763 & 0.581 & 0.236 &  & 0.28 & 0.614 & 0.466 & 0.154 & 0.923 & 0.299 & 0.639 \\
Jurassic Grande (17B) & 0.233 & 0.709 & 0.58 & 0.183 &  & 0.268 & 0.58 & 0.472 & 0.148 & 0.943 & 0.715 & 0.632 \\
Jurassic Large (7.5B) & 0.236 & 0.68 & 0.524 & 0.152 &  & 0.224 & 0.528 & 0.444 & 0.154 & 0.947 & 0.679 & 0.514 \\
Anthropic-LM (52B) & 0.461 & 0.816 & 0.644 & 0.235 & 0.62 & 0.354 &  &  & 0.277 & 0.925 & 0.458 & 0.657 \\
BLOOM (176B) & 0.268 & 0.729 & 0.585 & 0.193 & 0.389 & 0.275 & 0.585 & 0.48 & 0.173 & 0.94 & 0.529 & 0.552 \\
T0++ (11B) & 0.395 & 0.562 & 0.227 & 0.078 & 0.485 & 0.093 &  &  & 0.298 & 0.548 & 0.631 & 0.398 \\
Cohere xlarge & 0.307 & 0.755 & 0.562 & 0.252 & 0.326 & 0.288 & 0.66 & 0.47 & 0.159 & 0.934 & 0.283 & 0.57 \\
Cohere large & 0.27 & 0.722 & 0.528 & 0.177 & 0.393 & 0.264 & 0.575 & 0.446 & 0.209 & 0.918 & 0.164 & 0.577 \\
Cohere medium & 0.273 & 0.609 & 0.455 & 0.126 & 0.242 & 0.202 & 0.525 & 0.42 & 0.171 & 0.864 & 0.199 & 0.502 \\
Cohere small & 0.197 & 0.44 & 0.178 & 0.054 & 0.152 & 0.145 & 0.308 & 0.28 & 0.164 & 0.501 & 0.802 & 0.455 \\
GPT-J (6B) & 0.214 & 0.538 & 0.439 & 0.138 & 0.327 & 0.239 & 0.487 & 0.412 & 0.167 & 0.946 & 0.251 & 0.6 \\
GPT-NeoX (20B) & 0.207 & 0.685 & 0.458 & 0.162 & 0.345 & 0.246 & 0.556 & 0.446 & 0.159 & 0.933 & 0.189 & 0.484 \\
T5 (11B) & 0.215 & 0.812 & 0.05 & 0.154 & 0.239 & 0.073 &  &  & 0.078 & 0.345 & 0.424 & 0.325 \\
UL2 (20B) & 0.216 & 0.773 & 0.054 & 0.133 & 0.146 & 0.109 &  &  & 0.164 & 0.36 & 0.385 & 0.28 \\
OPT (66B) & 0.226 & 0.736 & 0.528 & 0.222 & 0.316 & 0.269 & 0.597 & 0.454 & 0.19 & 0.915 & 0.192 & 0.55 \\
OPT (175B) & 0.299 & 0.795 & 0.566 & 0.247 & 0.377 & 0.28 & 0.66 & 0.5 & 0.173 & 0.945 & 0.193 & 0.586 \\
GPT-3 (175B) & 0.398 & 0.716 & 0.608 & 0.273 & 0.311 & 0.279 & 0.641 & 0.502 & 0.148 & 0.905 & 0.23 & 0.63 \\
GPT-3 (6.7B) & 0.224 & 0.611 & 0.499 & 0.145 & 0.299 & 0.243 & 0.522 & 0.43 & 0.19 & 0.888 & 0.187 & 0.457 \\
GPT-3 (1.3B) & 0.201 & 0.444 & 0.378 & 0.087 & 0.229 & 0.196 & 0.401 & 0.326 & 0.171 & 0.501 & 0.591 & 0.461 \\
GPT-3 (350M) & 0.211 & 0.584 & 0.204 & 0.061 & 0.214 & 0.153 & 0.294 & 0.318 & 0.188 & 0.873 & 0.621 & 0.359 \\
Davinci Instruct v2 & 0.548 & 0.844 & 0.651 & 0.327 & 0.609 & 0.357 & 0.703 & 0.54 & 0.546 & 0.943 & 0.384 & 0.62 \\
Curie Instruct & 0.248 & 0.592 & 0.465 & 0.128 & 0.319 & 0.269 & 0.534 & 0.452 & 0.176 & 0.905 & 0.613 & 0.466 \\
Babbage Instruct & 0.203 & 0.382 & 0.296 & 0.055 & 0.229 & 0.195 & 0.405 & 0.386 & 0.176 & 0.913 & 0.809 & 0.48 \\
Ada Instruct & 0.2 & 0.444 & 0.103 & 0.008 & 0.116 & 0.093 & 0.27 & 0.266 & 0.154 & 0.811 & 0.795 & 0.389 \\
GLM (130B) & 0.287 & 0.791 & 0.657 & 0.125 & 0.117 & 0.23 &  &  & 0.179 & 0.94 & 0.81 & 0.555 \\
YaLM (100B) & 0.201 & 0.569 & 0.146 & 0.1 & 0.16 & 0.094 &  &  & 0.098 & 0.766 & 0.705 & 0.409 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Counterfactual fairness based on perturbations for all models across all generic scenarios.}}
\label{tab:fairness-generic}
\end{table*}

==> tables/metrics/tasks_robustness.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
Adapter & MMLU  (EM) & BoolQ (EM) & NarrativeQA (F1) & NaturalQ (closed-book) (F1) & NaturalQ (open-book) (F1) & QuAC  (F1) & HellaSwag (EM) & OpenbookQA (EM) & TruthfulQA (EM) & IMDB (EM) & CivilComments (EM) & RAFT (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.216 & 0.356 & 0.546 & 0.17 &  & 0.227 & 0.726 & 0.43 & 0.154 & 0.876 & 0.283 & 0.557 \\
Jurassic Grande (17B) & 0.231 & 0.519 & 0.513 & 0.157 &  & 0.232 & 0.695 & 0.424 & 0.135 & 0.907 & 0.576 & 0.498 \\
Jurassic Large (7.5B) & 0.216 & 0.474 & 0.428 & 0.105 &  & 0.199 & 0.646 & 0.412 & 0.13 & 0.914 & 0.694 & 0.445 \\
Anthropic-LM (52B) & 0.437 & 0.657 & 0.663 & 0.234 & 0.6 & 0.322 &  &  & 0.324 & 0.87 & 0.475 & 0.568 \\
BLOOM (176B) & 0.245 & 0.561 & 0.563 & 0.193 & 0.352 & 0.24 & 0.699 & 0.438 & 0.168 & 0.902 & 0.549 & 0.495 \\
T0++ (11B) & 0.382 & 0.38 & 0.232 & 0.082 & 0.452 & 0.092 &  &  & 0.323 & 0.35 & 0.52 & 0.393 \\
Cohere xlarge & 0.287 & 0.527 & 0.389 & 0.223 & 0.24 & 0.237 & 0.759 & 0.448 & 0.153 & 0.883 & 0.253 & 0.518 \\
Cohere large & 0.257 & 0.462 & 0.371 & 0.155 & 0.26 & 0.213 & 0.687 & 0.43 & 0.202 & 0.861 & 0.134 & 0.489 \\
Cohere medium & 0.219 & 0.416 & 0.309 & 0.103 & 0.175 & 0.156 & 0.651 & 0.382 & 0.174 & 0.734 & 0.069 & 0.395 \\
Cohere small & 0.203 & 0.309 & 0.087 & 0.025 & 0.058 & 0.106 & 0.405 & 0.238 & 0.168 & 0.273 & 0.656 & 0.4 \\
GPT-J (6B) & 0.21 & 0.32 & 0.145 & 0.105 & 0.063 & 0.156 & 0.619 & 0.398 & 0.165 & 0.909 & 0.226 & 0.502 \\
GPT-NeoX (20B) & 0.19 & 0.458 & 0.424 & 0.133 & 0.298 & 0.209 & 0.663 & 0.414 & 0.151 & 0.89 & 0.187 & 0.4 \\
T5 (11B) & 0.242 & 0.656 & 0.048 & 0.152 & 0.174 & 0.071 &  &  & 0.127 & 0.295 & 0.482 & 0.3 \\
UL2 (20B) & 0.23 & 0.605 & 0.061 & 0.111 & 0.142 & 0.112 &  &  & 0.165 & 0.339 & 0.503 & 0.27 \\
OPT (66B) & 0.206 & 0.521 & 0.411 & 0.195 & 0.205 & 0.212 & 0.699 & 0.45 & 0.194 & 0.86 & 0.114 & 0.398 \\
OPT (175B) & 0.284 & 0.559 & 0.415 & 0.195 & 0.191 & 0.217 & 0.744 & 0.488 & 0.179 & 0.893 & 0.064 & 0.468 \\
GPT-3 (175B) & 0.35 & 0.543 & 0.502 & 0.263 & 0.25 & 0.22 & 0.738 & 0.474 & 0.142 & 0.837 & 0.193 & 0.511 \\
GPT-3 (6.7B) & 0.194 & 0.404 & 0.357 & 0.127 & 0.213 & 0.189 & 0.632 & 0.396 & 0.179 & 0.809 & 0.191 & 0.391 \\
GPT-3 (1.3B) & 0.172 & 0.281 & 0.265 & 0.068 & 0.138 & 0.158 & 0.489 & 0.314 & 0.15 & 0.271 & 0.607 & 0.423 \\
GPT-3 (350M) & 0.193 & 0.32 & 0.1 & 0.024 & 0.038 & 0.099 & 0.37 & 0.27 & 0.156 & 0.777 & 0.618 & 0.325 \\
Davinci Instruct v2 & 0.531 & 0.771 & 0.654 & 0.306 & 0.619 & 0.31 & 0.776 & 0.52 & 0.573 & 0.91 & 0.564 & 0.63 \\
Curie Instruct & 0.228 & 0.416 & 0.335 & 0.121 & 0.262 & 0.187 & 0.625 & 0.424 & 0.179 & 0.838 & 0.135 & 0.395 \\
Babbage Instruct & 0.185 & 0.201 & 0.121 & 0.04 & 0.138 & 0.093 & 0.468 & 0.39 & 0.156 & 0.856 & 0.809 & 0.386 \\
Ada Instruct & 0.194 & 0.245 & 0.049 & 0.005 & 0.081 & 0.069 & 0.32 & 0.248 & 0.144 & 0.7 & 0.791 & 0.327 \\
GLM (130B) & 0.307 & 0.645 & 0.681 & 0.121 & 0.109 & 0.223 &  &  & 0.191 & 0.904 & 0.81 & 0.568 \\
YaLM (100B) & 0.12 & 0.208 & 0.102 & 0.031 & 0.093 & 0.091 &  &  & 0.086 & 0.65 & 0.738 & 0.191 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Robustness to semantics-preserving perturbations for all models across all generic scenarios.}}
\label{tab:robustness-generic}
\end{table*}

==> tables/metrics/tasks_toxicity.tex <==
\begin{table}[htp]
\resizebox{.5\textwidth}{!}{
\begin{tabular}{lrr}
\toprule
Adapter & CNN/DailyMail (Toxic fraction) & XSUM (Toxic fraction) \\
\midrule
Jurassic Jumbo (178B) & 0.004 & 0.002 \\
Jurassic Grande (17B) & 0.002 & 0.002 \\
Jurassic Large (7.5B) & 0.004 & 0.002 \\
Anthropic-LM (52B) & 0.004 & 0.002 \\
BLOOM (176B) & 0.002 &  \\
T0++ (11B) & 0.002 & 0.004 \\
Cohere xlarge & 0.002 & 0.002 \\
Cohere large & 0.004 & 0.002 \\
Cohere medium & 0.002 &  \\
Cohere small & 0.004 &  \\
GPT-J (6B) & 0.002 &  \\
GPT-NeoX (20B) & 0.002 & 0.004 \\
T5 (11B) & 0.002 &  \\
UL2 (20B) & 0.006 &  \\
OPT (66B) & 0.002 & 0.002 \\
OPT (175B) & 0.002 & 0.004 \\
GPT-3 (175B) & 0.006 & 0.002 \\
GPT-3 (6.7B) & 0.004 &  \\
GPT-3 (1.3B) & 0.002 &  \\
GPT-3 (350M) & 0.004 &  \\
Davinci Instruct v2 & 0.004 & 0.002 \\
Curie Instruct &  & 0.002 \\
Babbage Instruct &  &  \\
Ada Instruct &  &  \\
GLM (130B) &  &  \\
YaLM (100B) &  & 0.002 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Toxicity of model generations according to PerspectiveAPI for all models across all generic scenarios.}}
\label{tab:toxicity-generic}
\end{table}

==> tables/models-abridged.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Model & Model Creator & \# Parameters & Access & Release date \\
\midrule
% AI21 (3) (1)
\jurassicjumbo & AI21 Labs  & 178B & commercial & August 11, 2021\\
% Date source: https://www.businesswire.com/news/home/20210811005033/en/AI21-Labs-Makes-Language-AI-Applications-Accessible-to-Broader-Audience
\jurassicgrande & AI21 Labs  & 17B & commercial & May 3, 2022\\
% Date source: https://twitter.com/AI21Labs/status/1521421819395379201
\jurassiclarge & AI21 Labs  & 7.5B & commercial & August 11, 2021\\
% Date source: https://www.businesswire.com/news/home/20210811005033/en/AI21-Labs-Makes-Language-AI-Applications-Accessible-to-Broader-Audience
\midrule
% Anthropic (1) (1)
\anthropic & Anthropic  & 52B & private & December 1, 2021 \\
% Date source: https://arxiv.org/abs/2112.00861
\midrule
% BigScience (2) (2)
\bloom & BigScience  & 176B & public & June 28, 2022\\
% Date source: https://twitter.com/BigScienceLLM/status/1541828788375486469
\tzero & BigScience  & 11B & public & October 15, 2021 \\
% Date source: https://arxiv.org/abs/2110.08207
\midrule
% Cohere (4) (1)
\coherexl & Cohere  & Unknown & commercial & April 25, 2022 \\
% Date source: https://docs.cohere.ai/release-notes/
\coherel & Cohere  & Unknown & commercial & March 29, 2022 \\
% Date source: https://docs.cohere.ai/release-notes/
\coherem & Cohere  & Unknown & commercial & March 29, 2022 \\
% Date source: https://docs.cohere.ai/release-notes/
\coheres & Cohere  & Unknown & commercial & March 29, 2022\\
% Date source: https://docs.cohere.ai/release-notes/
\midrule
% EleutherAI (2) (2)
\gptj & EleutherAI  & 6B & public & June 4, 2021\\
% Date source: https://arankomatsuzaki.wordpress.com/2021/06/04/gpt-j/
\gptneox & EleutherAI  & 20B & public & February 2, 2022 \\
% Date source: https://www.eleuther.ai/projects/gpt-neox/
\midrule
% Google (2) (2)
\tfive & Google  & 11B & public & October 23, 2019 \\
% Date source: https://arxiv.org/abs/1910.10683
\ultwo & Google  & 20B & public & May 10, 2022\\
% Date source: https://arxiv.org/abs/2205.05131
\midrule
% Meta (2) (1)
\optsixsix & Meta  & 66B & public & May 2, 2022\\
% Date source: https://arxiv.org/abs/2205.01068
\optonesevenfive & Meta  & 175B & public & May 2, 2022\\
% Date source: https://arxiv.org/abs/2205.01068
\midrule
% Microsoft (1) (1)
\mtnlgseven & Microsoft/NVIDIA  & 7B & private & January 28, 2022 \\
% Date source: https://arxiv.org/abs/2201.11990
\mtnlgfivethreezero & Microsoft/NVIDIA  & 530B & private & January 28, 2022 \\
% Date source: https://arxiv.org/abs/2201.11990
\midrule
% OpenAI (10) (3)
\gptdavinci & OpenAI  & 175B & commercial & May 28, 2020 \\
% Date souce: https://arxiv.org/abs/2005.14165
\gptcurie & OpenAI  & 6.7B & commercial & May 28, 2020\\
% Date souce: https://arxiv.org/abs/2005.14165
\gptbabbage & OpenAI  & 1.3B & commercial & May 28, 2020\\
% Date souce: https://arxiv.org/abs/2005.14165
\gptada & OpenAI  & 350M & commercial & May 28, 2020\\
% Date souce: https://arxiv.org/abs/2005.14165
\instructdavinci & OpenAI  & Unknown & commercial & Unknown\\
\instructcurie & OpenAI  & Unknown & commercial & Unknown\\
\instructbabbage & OpenAI  & Unknown & commercial & Unknown\\
\instructada & OpenAI  & Unknown & commercial & Unknown\\
\davincicodex & OpenAI  & Unknown & commercial & Unknown\\
\cushmancodex & OpenAI  & Unknown & commercial & Unknown\\
\midrule
% Tsinghua University (1) (1)
\glm & Tsinghua University  & 130B & public & August 4, 2022\\
% Date source: https://keg.cs.tsinghua.edu.cn/glm-130b/posts/glm-130b/
\midrule
% Yandex (1) (1)
\yalm & Yandex  & 100B & public & June 23, 2022\\
% Date source: https://medium.com/yandex/yandex-publishes-yalm-100b-its-the-largest-gpt-like-neural-network-in-open-source-d1df53d0e9a6
\bottomrule
\end{tabular}}
\caption{\textbf{Models.} Description of the \nummodels models evaluated in this effort.}
\label{tab:models}
\end{table*}

==> tables/tasks/miscellaneous_text_classification_accuracy.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lr}
\toprule
Adapter & RAFT (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.702 \\
Jurassic Grande (17B) & 0.664 \\
Jurassic Large (7.5B) & 0.536 \\
Anthropic-LM (52B) & 0.68 \\
BLOOM (176B) & 0.584 \\
T0++ (11B) & 0.411 \\
Cohere xlarge & 0.602 \\
Cohere large & 0.609 \\
Cohere medium & 0.523 \\
Cohere small & 0.509 \\
GPT-J (6B) & 0.616 \\
GPT-NeoX (20B) & 0.511 \\
T5 (11B) & 0.336 \\
UL2 (20B) & 0.293 \\
OPT (66B) & 0.575 \\
OPT (175B) & 0.6 \\
GPT-3 (175B) & 0.655 \\
GPT-3 (6.7B) & 0.484 \\
GPT-3 (1.3B) & 0.491 \\
GPT-3 (350M) & 0.386 \\
Davinci Instruct v2 & 0.691 \\
Curie Instruct & 0.495 \\
Babbage Instruct & 0.53 \\
Ada Instruct & 0.423 \\
GLM (130B) & 0.593 \\
YaLM (100B) & 0.555 \\
\bottomrule
\end{tabular}}
\caption{Results for text classifications (miscellaneous)}
\label{fig:accuracy (miscellaneous_text_classification)}
\end{table}

==> tables/tasks/question_answering_accuracy.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrr}
\toprule
Adapter & MMLU (EM) & BoolQ (EM) & NarrativeQA (F1) & NaturalQ (closed-book) (F1) & NaturalQ (open-book) (F1) & QuAC (F1) & HellaSwag (EM) & OpenbookQA (EM) & TruthfulQA (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.256 & 0.791 & 0.688 & 0.288 &  & 0.365 & 0.765 & 0.534 & 0.177 \\
Jurassic Grande (17B) & 0.276 & 0.727 & 0.691 & 0.226 &  & 0.372 & 0.739 & 0.52 & 0.173 \\
Jurassic Large (7.5B) & 0.265 & 0.712 & 0.634 & 0.197 &  & 0.304 & 0.7 & 0.514 & 0.19 \\
Anthropic-LM (52B) & 0.502 & 0.829 & 0.718 & 0.28 & 0.672 & 0.449 &  &  & 0.375 \\
BLOOM (176B) & 0.281 & 0.745 & 0.671 & 0.227 & 0.456 & 0.358 & 0.744 & 0.532 & 0.199 \\
T0++ (11B) & 0.413 & 0.592 & 0.355 & 0.096 & 0.604 & 0.154 &  &  & 0.336 \\
Cohere xlarge & 0.341 & 0.784 & 0.647 & 0.299 & 0.394 & 0.368 & 0.81 & 0.55 & 0.196 \\
Cohere large & 0.309 & 0.744 & 0.641 & 0.227 & 0.472 & 0.343 & 0.736 & 0.542 & 0.211 \\
Cohere medium & 0.307 & 0.643 & 0.578 & 0.176 & 0.331 & 0.284 & 0.706 & 0.496 & 0.185 \\
Cohere small & 0.247 & 0.481 & 0.31 & 0.074 & 0.234 & 0.213 & 0.483 & 0.348 & 0.185 \\
GPT-J (6B) & 0.267 & 0.544 & 0.547 & 0.165 & 0.412 & 0.319 & 0.663 & 0.512 & 0.191 \\
GPT-NeoX (20B) & 0.273 & 0.72 & 0.605 & 0.2 & 0.446 & 0.342 & 0.718 & 0.53 & 0.193 \\
T5 (11B) & 0.295 & 0.831 & 0.086 & 0.189 & 0.29 & 0.119 &  &  & 0.179 \\
UL2 (20B) & 0.241 & 0.806 & 0.092 & 0.17 & 0.191 & 0.154 &  &  & 0.199 \\
OPT (66B) & 0.258 & 0.757 & 0.652 & 0.26 & 0.438 & 0.35 & 0.745 & 0.534 & 0.219 \\
OPT (175B) & 0.32 & 0.816 & 0.671 & 0.291 & 0.458 & 0.365 & 0.791 & 0.586 & 0.248 \\
GPT-3 (175B) & 0.42 & 0.734 & 0.697 & 0.334 & 0.376 & 0.355 & 0.775 & 0.586 & 0.2 \\
GPT-3 (6.7B) & 0.242 & 0.642 & 0.594 & 0.207 & 0.376 & 0.319 & 0.682 & 0.502 & 0.237 \\
GPT-3 (1.3B) & 0.219 & 0.502 & 0.516 & 0.117 & 0.307 & 0.273 & 0.555 & 0.438 & 0.187 \\
GPT-3 (350M) & 0.256 & 0.61 & 0.333 & 0.086 & 0.304 & 0.226 & 0.435 & 0.38 & 0.22 \\
Davinci Instruct v2 & 0.574 & 0.863 & 0.748 & 0.388 & 0.68 & 0.445 & 0.815 & 0.594 & 0.633 \\
Curie Instruct & 0.259 & 0.616 & 0.569 & 0.169 & 0.403 & 0.376 & 0.676 & 0.514 & 0.202 \\
Babbage Instruct & 0.229 & 0.394 & 0.429 & 0.076 & 0.33 & 0.274 & 0.561 & 0.452 & 0.203 \\
Ada Instruct & 0.25 & 0.509 & 0.218 & 0.016 & 0.205 & 0.177 & 0.429 & 0.346 & 0.196 \\
GLM (130B) & 0.321 & 0.839 & 0.739 & 0.153 & 0.163 & 0.292 &  &  & 0.209 \\
YaLM (100B) & 0.267 & 0.648 & 0.536 & 0.14 & 0.375 & 0.307 &  &  & 0.229 \\
\bottomrule
\end{tabular}}
\caption{Results for question answering}
\label{fig:accuracy (question_answering)}
\end{table*}

==> tables/tasks/sentiment_analysis_accuracy.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lr}
\toprule
Adapter & IMDB (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.927 \\
Jurassic Grande (17B) & 0.949 \\
Jurassic Large (7.5B) & 0.952 \\
Anthropic-LM (52B) & 0.93 \\
BLOOM (176B) & 0.944 \\
T0++ (11B)☠ & 0.57 \\
Cohere xlarge & 0.938 \\
Cohere large & 0.925 \\
Cohere medium & 0.886 \\
Cohere small & 0.521 \\
GPT-J (6B) & 0.953 \\
GPT-NeoX (20B) & 0.945 \\
T5 (11B) & 0.382 \\
UL2 (20B) & 0.403 \\
OPT (66B) & 0.921 \\
OPT (175B) & 0.948 \\
GPT-3 (175B) & 0.913 \\
GPT-3 (6.7B) & 0.902 \\
GPT-3 (1.3B) & 0.52 \\
GPT-3 (350M) & 0.898 \\
Davinci Instruct v2 & 0.947 \\
Curie Instruct & 0.915 \\
Babbage Instruct & 0.923 \\
Ada Instruct & 0.839 \\
GLM (130B) & 0.955 \\
YaLM (100B) & 0.8 \\
\bottomrule
\end{tabular}}
\caption{Results for sentiment analysis}
\label{fig:accuracy (sentiment_analysis)}
\end{table}

==> tables/tasks/summarization_accuracy.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lrr}
\toprule
Adapter & CNN/DailyMail (ROUGE-2) & XSUM (ROUGE-2) \\
\midrule
Jurassic Jumbo (178B) & 0.149 & 0.122 \\
Jurassic Grande (17B) & 0.152 & 0.117 \\
Jurassic Large (7.5B) & 0.13 & 0.103 \\
Anthropic-LM (52B) & 0.155 & 0.126 \\
BLOOM (176B) & 0.113 & 0.032 \\
T0++ (11B)☠ & 0.121 & 0.106 \\
Cohere xlarge & 0.166 & 0.128 \\
Cohere large & 0.15 & 0.102 \\
Cohere medium & 0.129 & 0.085 \\
Cohere small & 0.08 & 0.027 \\
GPT-J (6B) & 0.143 & 0.095 \\
GPT-NeoX (20B) & 0.145 & 0.095 \\
T5 (11B) & 0.054 & 0.017 \\
UL2 (20B) & 0.053 & 0.05 \\
OPT (66B) & 0.147 & 0.122 \\
OPT (175B) & 0.167 & 0.156 \\
GPT-3 (175B) & 0.148 & 0.139 \\
GPT-3 (6.7B) & 0.137 & 0.103 \\
GPT-3 (1.3B) & 0.125 & 0.02 \\
GPT-3 (350M) & 0.107 & 0.003 \\
Davinci Instruct v2 & 0.163 & 0.146 \\
Curie Instruct & 0.157 & 0.075 \\
Babbage Instruct & 0.161 & 0.047 \\
Ada Instruct & 0.134 & 0.033 \\
GLM (130B) & 0.153 & 0.136 \\
YaLM (100B) & 0.022 & 0.022 \\
\bottomrule
\end{tabular}}
\caption{Results for summarization}
\label{fig:accuracy (summarization)}
\end{table}

==> tables/tasks/toxicity_detection_accuracy.tex <==
\begin{table}[htp]
\resizebox{.45\textwidth}{!}{
\begin{tabular}{lr}
\toprule
Adapter & CivilComments (EM) \\
\midrule
Jurassic Jumbo (178B) & 0.407 \\
Jurassic Grande (17B) & 0.788 \\
Jurassic Large (7.5B) & 0.777 \\
Anthropic-LM (52B) & 0.589 \\
BLOOM (176B) & 0.614 \\
T0++ (11B) & 0.672 \\
Cohere xlarge & 0.389 \\
Cohere large & 0.277 \\
Cohere medium & 0.212 \\
Cohere small & 0.805 \\
GPT-J (6B) & 0.284 \\
GPT-NeoX (20B) & 0.224 \\
T5 (11B) & 0.604 \\
UL2 (20B) & 0.62 \\
OPT (66B) & 0.198 \\
OPT (175B) & 0.215 \\
GPT-3 (175B) & 0.294 \\
GPT-3 (6.7B) & 0.337 \\
GPT-3 (1.3B) & 0.646 \\
GPT-3 (350M) & 0.662 \\
Davinci Instruct v2 & 0.688 \\
Curie Instruct & 0.679 \\
Babbage Instruct & 0.809 \\
Ada Instruct & 0.799 \\
GLM (130B) & 0.81 \\
YaLM (100B) & 0.753 \\
\bottomrule
\end{tabular}}
\caption{Results for toxicity detection}
\label{fig:accuracy (toxicity_detection)}
\end{table}
